The ionised gas outflow in the Circinus galaxy: kinematics and physical conditions

We employ MUSE/VLT data to study the ionised and highly ionised gas phases of the feedback in Circinus, the closest Seyfert 2 galaxy to us. The analysis of the nebular emission allowed us to detect a remarkable high-ionisation gas outflow beyond the galaxy plane traced by the coronal lines [Fe VII] $\lambda$6089 and [Fe X] $\lambda$6374, extending up to 700 pc and 350 pc NW from the nucleus, respectively. This is the first time that the [Fe X] emission is observed at such distances from the central engine in an AGN. The gas kinematics reveals expanding gas shells with velocities of a few hundred km s$^{-1}$, spatially coincident with prominent hard X-ray emission detected by Chandra. Density and temperature sensitive line ratios show that the extended high-ionisation gas is characterized by a temperature reaching 25000 K and an electron density > 10$^2$ cm$^{-3}$. We found that local gas excitation by shocks produced by the passage of a radio jet leads to the spectacular high-ionisation emission in this object. This hypothesis is fully supported by photoionisation models that accounts for the combined effects of the central engine and shocks. They reproduce the observed emission line spectrum at different locations inside and outside of the NW ionisation cone. The energetic outflow produced by the radio jet is spatially located close to an extended molecular outflow recently reported using ALMA which suggests that they both represent different phases of the same feedback process acting on the AGN.

==> doc/latex/amscls/README <==
README file for AMS document classes amsart/book/proc 2.20.5 [2020/05/21]

Copyright 2004, 2010, 2014-2017, 2020 American Mathematical Society.

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3c
of this license or (at your option) any later version.
The latest version of this license is in
  http://www.latex-project.org/lppl.txt
and version 1.3c or later is part of all distributions of LaTeX
version 2005/12/01 or later.

This work has the LPPL maintenance status `maintained'.

The Current Maintainer of this work is the American Mathematical
Society.

American Mathematical Society
Technical Support
Publications Technical Group
201 Charles Street
Providence, RI 02904
USA
tel: (401) 455-4080
     (800) 321-4267 (USA and Canada only)
fax: (401) 331-3842
email: tech-support@ams.org

========================================================================

See manifest.txt for a list of all the files in the distribution.

The document classes amsart, amsbook, amsproc and related packages are
provided by the American Mathematical Society for authors to use with
LaTeX.  They produce the overall layout and appearance of AMS
publications.

In order to use an AMS document class you need to have TeX software
installed first.  TeX is not an AMS product. If you need information
on getting TeX see one of the following:

  http://www.tug.org/
  https://www.ams.org/tex/tex-resources.html

User documentation for the AMS document classes is contained in the
class-specific AMS Author Handbook, found at these locations:

  https://www.ams.org/tex/author-handbook  (individual handbooks)
  http://mirror.ctan.org/tex-archive/info/amscls-doc.zip  (full source)

Additional documentation for the AMS document classes and the related
theorem package is found in

  diffs-c.txt
  amsthdoc.pdf
  thmtest.tex
  thmtest.pdf

which are included in the collection.  Answers to some specific
questions can be found in the AMS Author FAQ:

  https://www.ams.org/tex/amsclass-faq.html

The recommended procedure for making a custom document class based on an
AMS class is to make a copy of the relevant .cls file using a different
name and edit the copy---e.g., copy amsbook.cls to mybook.cls.  (In
general we advise against using \LoadClass, unless the base class is
frozen or changes to the base class are under your control.)

========================================================================
RECENT CHANGES

---amsclass.dtx 2.20.5 2020/05/21
Added support for MSC 2020 and made it the default.

---amsclass.dtx 2.20.4 2017/10/31
Changed \emailaddrname: replaced "E-mail" by "Email"

---amsclass.dtx 2.20.3 2017/10/06
Don't assume amsfonts is available when providing a fallback
definition of \dh; instead, issue a warning and substitute "dh".

---documentation files 2017/11/15
instr-l.* removed; superseded by (class-specific) AMS Author Handbooks
at https://www.ams.org/tex/author-handbook
or http://mirror.ctan.org/tex-archive/info/amscls-doc.zip

========================================================================
PREVIOUS CHANGES

---amsthdoc.tex 2.20.2 2015/04/10
Completely rewritten, adding examples, workarounds, and notes on
interaction with other packages and document classes.

---amsclass.dtx 2.20.2 2015/03/10
Patched definition of \[ for compatibility with the fixltx2e package
and post-2014 versions of the LaTeX kernel.  Thanks to David Carlisle.

---amsclass.ins 2.25 2014/07/24
   amsmidx.ins  1.1  2014/07/24
   upref.ins    1.1  2014/07/24
Superseded ams-c1.ins by individual .ins files per .dtx file

---amsbooka.dtx 2.08 2014/07/11
1. When chapter has an author, reset running heads to be author/left,
   chapter title/right.
2. Added \barefootnote and inchapterbibliography.
3. Added (optional) \copyrightinfo per chapter.

---amsclass.dtx 2.20.1 2009/07/02
1. Added [2010] option as permissible year for \subjclass.
2. Revised header block to explicitly recognize the LPPL.

---ams-c1.ins 2.20 2004/08/03
Added amsmidx package.

---amsclass.dtx 2.20 2004/08/06
1. Added facility for additional line(s) in copyright block.
2. Corrected handling of section heading with no title.
3. Got rid of spurious "Appendix" in t-of-c in \backmatter.
4. Changed MR number formatting to use new style as on MathSciNet.
5. Created commands for various style elements and substituted them
   for hard-coded values to simplify building derived classes.
6. Added sectioning and otherwise cleaned up commentary.

---amsclass.faq - 2004/08/06
Removed from distribution; replaced by on-line FAQ at
http://www.ams.org/tex/amsclass-faq.html

---amsdtx.dtx 2.06 2004/08/06
1. Reworked indexing commands for compatibility with doc.sty.
2. Added option environment for enhanced indexing.
3. Improved formatting.

---amsthdoc.tex 2.20 2004/08/03
1. Substantially rewritten for clarity.
2. Added documentation for \newtheoremstyle.

---instr-l.tex 2.20 2004/08/05
Substantially rewritten for clarity and to add instructions for new
features; see note on amsclass.dtx regarding features.

---mrabbrev.bib - 2004/08/05
Removed from distribution; this is now available separately from
http://www.ams.org/tools/mrabbrev.bib 

---thmtest.tex 2.01 2004/08/02
1. Corrected counter for theorems with switched headers.
2. Added section headings for clarity.
3. Added example ending with a display and \qedhere.

---upref.dtx 2.01 2004/07/29
1. Added code to make package work with hyperref.
2. Improved documentation.

---amsclass.dtx 2.14 2004/04/26 (not released)
1. Incorporated pending changes left by Michael Downes:
  - Added trap in headings in case \thanks was set within \author,
    and added \thanks@warning.
  - Cleaned up and completed unfinished documentation.
2. Added braces in \uppercasenonmath to limit scope.
3. Added \contrib mechanism to handle "non-author" authors.
4. Segregated definitions of administrative footnotes to permit easier
   customization for AMS journals.
5. Added explicit \bibliofont to permit easy change for special uses.
6. Changed MR number formatting to correspond to new access numbers
   used by MathSciNet.
7. Added \@citestyle and \citeform to simplify font changes in citations.
8. Added OT1 defaults for \DH, \dh, \DJ, \dj, required for author names.
9. Added \markleft to permit changing of only left running head

---amsclass.dtx 2.13 2002/12/04 (not released)
1. Fixed handling of theorem head punctuation with \swapnumbers.
2. Changed \proofname to \providecommand in case it's already defined.
3. Made \small, \Small, etc., robust.
4. Better spacing in \l@figure to prevent overprinting of figure number.
5. Changed handling of author names to prevent internal line breaks.
6. Added \@noparitemfalse in \dth@everypar to prevent weird results in
   certain (rare) kinds of usage.
7. Some other cosmetic changes.

---amsthdoc.tex 2.02 2000/06/06
Use article class instead of amsldoc (which is overkill).

---amsldoc.cls - 2000/06/06
Removed from distribution, no longer needed by amsthdoc.

---amsclass.dtx 2.07 2000/06/05
Guard against \\ in argument of \author.

---amsclass.dtx 2.06 2000/06/02
Avoid using \@elt in qed stack because LaTeX output routine falls over
if triggered when something else is using \@elt.

---amsclass.dtx 2.05 2000/05/16
1. Added \indexintro.
2. Fixed erroneous init for thm@preskip, thm@postskip.

---amsclass.dtx 2.04 2000/03/10
\newtoks fix for old versions of LaTeX. Added some commentary about \cal.

---amsclass.dtx 2.03 2000/01/17
1. Removed dependency on amsgen package.
2. Added a warning about graphics for the draft option.
3. Improved qedhere handling for article/amsthm combination.

---amsclass.dtx 2.02 2000/01/17
Some fixes for the fleqn/qedhere case.
========================================================================

